Scheduling Two Agents on a Single Machine: A Parameterized Analysis of NP-hard Problems

Scheduling theory is an old and well-established area in combinatorial optimization, whereas the much younger area of parameterized complexity has only recently gained the attention of the community. Our aim is to bring these two areas closer together by studying the parameterized complexity of a class of single-machine two-agent scheduling problems. Our analysis focuses on the case where the number of jobs belonging to the second agent is considerably smaller than the number of jobs belonging to the first agent, and thus can be considered as a fixed parameter k. We study a variety of combinations of scheduling criteria for the two agents, and for each such combination we pinpoint its parameterized complexity with respect to the parameter k. The scheduling criteria that we analyze include the total weighted completion time, the total weighted number of tardy jobs, and the total weighted number of just-in-time jobs. Our analysis draws a borderline between tractable and intractable variants of these problems.

==> discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% Discussion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We would like to point out several directions for future research.
First,
while we determined the (parameterized) complexity of \textsc{Two Agent Scheduling}
when the input is given in binary,
our understanding of the complexity \textsc{Two Agent Scheduling} when the input is given in unary is lacking.
%most intriguingly,
%we do not know whether the problem is NP-hard.
%Another possible direction might be to consider the natural generalization of \textsc{Two Agent Scheduling}
%to an arbitrary number of clients.
Further,
it is natural to study \textsc{Two Agent Scheduling} when considering, e.g., other objective functions
or other, related, scheduling problems.

Finally,
we believe that our MILP formulation and the ideas underlying it,
as described in the proof of Theorem~\ref{theorem: unit weights},
might be useful for other problems.
We would like to see other problems which have a similar structure that might be utilized in similar ways.

==> dvir.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% RESULTS FOR FEW JOB TYPES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section,
we do not restrict the number $k$ of Bob's jobs,
but the number $t$ of types for his jobs.
Specifically,
we consider \textsc{Two Agent Scheduling} when all jobs are of unit weight
and there is only a small number $t$ of different processing times for Bob's jobs.
%In other words,
%we can group the jobs of Bob to $t$ groups,
%such that the jobs in each group have the same processing time.

\iffalse
We say that the schedule $\sigma_1$ \emph{dominates} the schedule $\sigma_2$,
if the sums of completion times for both Alice and Bob
(that is, $\sum_i w_i^A C_i^A$ and $\sum_i w_i^B C_i^A$),
are smaller or equal to the sums of completion times for them under $\sigma_2$
(as, in this case, $\sigma_1$ is better than $\sigma_2$ for both agents).
A \emph{Pareto point} is a schedule which is not dominated by any other schedule.
In what follows,
we will first prove that,
for the case of \textsc{Two Agent Scheduling} discussed above,
the number of Pareto points is polynomial in the input size,
and that it is possible to enumerate all of them in polynomial time.
We will get a polynomial-time algorithm by observing that it is enough to consider only the Pareto points.
\fi

Let us begin with the case of $t = 1$,
that is,
when all of Bob's jobs have the same processing time.
Fix a schedule $\sigma$
and consider two of Alice's jobs, $J_{i_1}^A$ and $J_{i_2}^A$,
where $i_1 < i_2$,
and therefore,
from the SPT (Shortest Processing Time first) rule,
also $p_{i_1}^A \leq p_{i_2}^A$.
Assume that there is one job $J_{j_1}^B$ of Bob
which is scheduled directly before $J_{i_1}^A$,
and another job $J_{j_2}^B$ of Bob
which is scheduled right after $J_{i_2}^A$.
Then,
perform the following \emph{pair-wise interchange} operation:
swap $J_{i_1}^A$ with $J_{j_1}^B$ and swap $J_{i_2}^A$ with $J_{j_2}^B$.
%
Notice that
  (1) the sum of completion times for Alice ($\sum_i w_i^A C_i^A$) did not change as a result of this pair-wise interchange operation,
  since all of Bob's jobs have the same processing time,
  and (2) the sum of completion times for Bob ($\sum_i w_i^B C_i^B$) might only improved,
  since $p_{i_1}^A \leq p_{i_2}^A$.
% Therefore, we have that the situation for both Alice and Bob did not deteriorate as a result of the pair-wise interchange operation.

Further,
after we exhaustively perform these pair-wise interchanges,
we reach a schedule which can concisely described as ``$a_1b_1a_2b_2a_3$'',
where $a_1 + a_2 + a_3 = n$,
$0 \leq a_2 \leq 1$,
and $b_1 + b_2 = k$,
with the intended meaning that $a_1$ of Alice's jobs are scheduled first,
then $b_1$ of Bob's jobs, than $a_2$ of Alice's jobs,
then $b_2$ of Bob's jobs, and finally $a_3$ of Alice's jobs.
To see why this representation defines a unique schedule,
recall the SPT (Shortest Processing Time first) rule.
A schedule in this form is called a schedule \emph{in normal-form}.
To see why we reach a schedule in normal-form after exhaustively performing pair-wise interchanges,
notice that it is possible to perform at least one pair-wise interchange operation
to any schedule $\sigma$ not in normal-form.

The above analysis suggests the following algorithm:
iterate over all possible $2nk$ schedules in normal-form,
and check whether at least one of them is feasible.
It is enough to consider only schedules in normal-form,
since if a schedule $\sigma$ which is feasible and not in normal-form exists,
then a schedule $\sigma'$ which is feasible and also in normal-form exists as well,
by exhaustively performing pair-wise interchanges on~$\sigma$.
%
We can generalize the above discussion to any number $t$ of types for Bob's jobs
to get the following result.

\begin{theorem}
\textsc{Two Agent Scheduling}
when the jobs of Alice and Bob are non-weighted
and Bob's jobs have a constant number $t$ of different processing times,
is solvable in polynomial time.
\end{theorem}

\begin{proof}
Let us group Bob's jobs into $t$ groups
by their processing times,
such that~$B_i$,
for $1 \leq i \leq t$,
denotes the set of Bob's jobs of the $i$th group.
Observe that the jobs of both Alice and Bob are sorted increasingly by their processing times,
as all jobs are non-weighted.
Let $J_{j_1}^{B_i}$ and $J_{j_2}^{B_i}$ be two jobs of the $i$th group,
where $J_{j_1}^{B_i}$ directly precedes a job $J_{i_1}^A$ of Alice
and
$J_{j_2}^{B_i}$ directly follows a job $J_{i_2}^A$ of Alice.
Swapping both these pairs leaves the sum of completion times for Alice unchanged,
as $J_{j_1}^{B_i}$ and $J_{j_2}^{B_i}$ have the same processing time,
and can only decrease the sum of completion times for Bob.

By doing so exhaustively for all job types of Bob we obtain a schedule which can be concisely described as
  ``$a_1b_1a_{1'}b_{1'}a_2b_2a_{2'}b_{2'}\cdots a_tb_ta_{t'}b_{t'}a_{\textrm{rest}}$'',
  where $a_{\textrm{rest}} + \sum_{i = 1}^t (a_i + a_{i'}) = n$,
  $0 \leq a_{i'} \leq 1$ for each $1 \leq i \leq t$,
  and $b_i + b_{i'} = |B_i|$ for each $1 \leq i \leq t$,
  with the intended meaning that $a_1$ of Alice's jobs are scheduled first,
  then $b_1$ of Bob's jobs of the first group,
  then $a_{1'}$ of Alice's jobs,
  then $b_{1'}$ of Bob's jobs of the first group,
  then $a_2$ of Alice's jobs,
  then $b_2$ of Bob's jobs of the second group,
  then $a_{2'}$ of Alice's jobs,
  then $b_{2'}$ of Bob's jobs of the second group,
  and so on,
  until, finally, $a_{\textrm{rest}}$ of Alice's jobs are scheduled.

Similarly to the above analysis for $t = 1$,
we have that it is enough to consider only schedules in this normal-form.
The number of normal-forms is upper-bounded by $k^t 2^t n^t$,
since it is uniquely defined by all possible values of $b_i$,
all possible (binary) values of $a_{i'}$,
and all possible values of $a_i$,
for $1 \leq i \leq t$.
%
Polynomial time algorithm then follows by iteratively checking all possible schedules in normal-form.
~\qed\end{proof}












\iffalse
\begin{theorem}
It is possible to enumerate all Pareto points
for \textsc{Two Agent Scheduling},
where the jobs of Alice and Bob are non-weighted and all of Bob's jobs have the same processing time,
in polynomial-time.
\end{theorem}

\begin{proof}
We will have some kind of a normal-form for schedules,
and show that it is enough to consider only schedules of this normal-form.
The number of schedules in normal-form will be shown to be polynomial in the input size,
and we will show how to generate all schedules of this normal-form.

To this end,
\fi



\iffalse
We now show that two different schedules in normal-form must have different sums of completion times for Agent A.
Towards a contradiction,
consider a smallest counter-example,
composed of the first schedule in normal-form, described via $P_1, P_2$ and $Q_1$,
and of the second schedule in normal-form, described via $P'_1, P'_2$ and $Q'_1$,
such that these normal-forms are different, but the sum of completion times for Agent A is the same for both schedules.
If both $P_1$ and $P'_1$ are non-empty, then, as job with the smallest processing time $J_1^A$ is contained
in $P_1$ and in $P'_1$, the example is not a smallest counter example.
Therefore, we can assume, without loss of generality,
that $P'_1$ is empty. The same arguments hold for $P_3$ and $P'_3$. As both schedules hold for the same set of jobs,
$P_3$ has to be the empty set.
But then, it is clear that the sum of completion times for Agent A is different in both schedules.
%
This finishes the proof,
and,
In fact,
we even showed that these normal-forms generate \emph{exactly} the Pareto points.
% ~\qed\end{proof}







The following Corollary follows easily,
by enumerating all normal-forms.

\begin{corollary}
\textsc{Two Agent Scheduling},
where the jobs of Alice and Bob are non-weighted and all of Bob's jobs have the same processing time,
is solvable in polynomial time.
\end{corollary}

\fi


==> introduction_old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% Introduction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Parameterized complexity facilitates the analysis of computational problems in terms of various instance parameters that may be independent of the total input length. In this way, problem instances are analyzed not only according to the total input length $n$, but also according to an additional numerical parameter $k$ that may encode other aspects of the input. A problem is considered tractable if there is an algorithm that optimally solves any instance in $f(k) \cdot n^{O(1)}$, where $f()$ is allowed to be any arbitrary computable function which is independent of $n$, and the exponent in $n^{O(1)}$ is required to be independent of $k$. For example, a running-time of $2^{O(k)} \cdot n ^3$ is considered tractable in the parameterized setting, while $n^k$ is not. In this way we can model scenarios where certain problem parameters are typically much smaller than the total input length, yet may not be small enough to be considered constant.

Parameterized complexity has enjoyed tremendous success since its first developments in the early 90s, as can be exemplified by the various textbooks on the subjects~\cite{Cygan2015,FG98,DF99,N06}. However, there has been certain concerns raised within the community regarding the many areas of computational sciences that the field has neglected. One of these is the area of scheduling, where currently there are less than a handful of papers~\cite{BodlaenderandFellows1995,FellowsandMcCartin2003,MnichandWiese2013,journals/scheduling/BevernMNW15,journals/corr/BevernNS15} dealing with scheduling problems from a parameterized perspective, with most of them focusing on those scheduling problems which can be represented as graph problems. In a typical scheduling problem, we are given a set of jobs that has to be scheduled on a set of machines, arranged according to a specific machine setting. The objective is to determine a schedule which minimizes a predefined scheduling criterion, such as the makespan, the total weighted completion time, and the total weighted tardiness. There are different machine settings such as a single machine, parallel machines, flow-shop and job-shop, and each scheduling problem may have different characteristics and constraints. The reader is referred to \emph{e.g.}~\cite{Brucker2006,Leung2004,Pinedo2008} for a comprehensive introduction to the area of scheduling.

The fact that there has been little research done on the parameterized complexity of scheduling problems is rather disappointing since scheduling problems seem to be particulary adequate for a parameterized analysis. For one, many scheduling problems are NP-hard, and thus most likely lack polynomial-time algorithms for finding optimal solutions. In several applications for such problems, an approximate solution results in big revenue losses, giving strong motivation for computing exact solutions even if computing such solutions requires a lot of resources. Moreover, scheduling problems typically have an abundance of natural problem parameters that can be comparatively small in practice; the number of different processing times, release times, due-dates, or the bound on the objective function are just a few examples. Thus, algorithms whose running times grow exponentially in such parameters alone should be quite useful in many scenarios arising in practice.

Our aim in this paper is to help close the gap between research in parameterized complexity and scheduling. We initiate a parameterized analysis on problems occurring in multi-agent scheduling~\cite{Agnetisbook}, a contemporary area which is nowadays at the cutting edge of scheduling research. We focus on the case where there are two agents, and all jobs are to be processed on a single machine. Furthermore, we focus on the situation where the second agent has a significantly smaller number of jobs than the other. The number of jobs belonging to this agent is thus taken as a parameter, and is denoted by $k$ throughout the paper.


\subsection{Our contribution}
\input{contribution}

\subsection{Related work}
\input{related_work} 
